Deep Animation Video Interpolation in the Wild

In the animation industry, cartoon videos are usually produced at low frame rate since hand drawing of such frames is costly and time-consuming. Therefore, it is desirable to develop computational models that can automatically interpolate the in-between animation frames. However, existing video interpolation methods fail to produce satisfying results on animation data. Compared to natural videos, animation videos possess two unique characteristics that make frame interpolation difficult: 1) cartoons comprise lines and smooth color pieces. The smooth areas lack textures and make it difficult to estimate accurate motions on animation videos. 2) cartoons express stories via exaggeration. Some of the motions are non-linear and extremely large. In this work, we formally define and study the animation video interpolation problem for the first time. To address the aforementioned challenges, we propose an effective framework, AnimeInterp, with two dedicated modules in a coarse-to-fine manner. Specifically, 1) Segment-Guided Matching resolves the "lack of textures" challenge by exploiting global matching among color pieces that are piece-wise coherent. 2) Recurrent Flow Refinement resolves the "non-linear and extremely large motion" challenge by recurrent predictions using a transformer-like architecture. To facilitate comprehensive training and evaluations, we build a large-scale animation triplet dataset, ATD-12K, which comprises 12,000 triplets with rich annotations. Extensive experiments demonstrate that our approach outperforms existing state-of-the-art interpolation methods for animation videos. Notably, AnimeInterp shows favorable perceptual quality and robustness for animation scenarios in the wild. The proposed dataset and code are available at https://github.com/lisiyao21/AnimeInterp/.

==> previous_version/intro_.tex <==
In animation industry, every frame of an anime video is hand drawn by painters.
% As a result, a large amount of human labor is consumed on creating similar contents, and the frame rate is set to 24 FPS. 
To reduce the budget, animation producers usually replicate one drawing for twice or three times. Such a reduction lowers the actual frame rate to 12 fps or even 8 fps, which narrowly meets the basic requirement for human eyes to regard discrete images as continuous. 
%
Therefore, it is promising to have a computational system to draw the intermediate cartoon frames automatically, with huge potentials to cut the cost and improve the user experience.

Video interpolation is a long existing topic drawing continuous attention in computer vision community. Recent methods take advantage of deep learning and can be roughly classified into two categories, \ie, the kernel-based and the flow-based. Kernel-based methods \cite{niklaus2017video,niklaus2017video2,lee2020adacof} learn a large size kernel for each pixel of the input and convolve the kernels with the input to synthesize the intermediate image. Flow-based methods \cite{jiang2018super,bao2019depth,niklaus2020softmax} generate the in-between frames by warping the input images with estimated optical flows. Although both types of methods have achieved great success in real-world video interpolation, there are sill many challenges to interpolate animation videos.

On the one hand, there is no animation dataset with sequential frames, and thus we can only train and evaluate existing interpolation methods on real-world datasets. However, as mentioned in \cite{chen2018cartoongan}, cartoon images are discriminative from the real-world images at least in three ways, namely, 1) clear contours for objects or semantic parts, 2) flat blocks filled with similar colors, and 3) less textures and shades. With such discrepancies, the performance on real-world videos cannot represent that on animations.

To benchmark interpolation methods, we collected a large-scale animation triplet dataset (ATD) for animation video interpolation. ATD consists of two parts, \ie, \trainset with 10,000 triplets for training and \testset with 2,000 triplets for test. In \testset, we also provide rich annotations for further analysis. Please see Section \ref{subsect:annotaion} for details.
One should note that it is difficult to collect such an dataset because we cannot simply divide sequential animation frames into triplets due to the unpredictable and irregular duplications. Instead, we combined human labors with auto selections to select triplets from over two million candidates. The establishment of ATD is elaborated in Section \ref{sect:animation_dataset}.

On the other hand, due to the low frame rate, animation videos usually come with larger motions than common videos. Moreover, certain actions of animation characters are intentionally exaggerated in pursuit of artistic effects. 
Such considerable motions are formidable for existing video interpolation methods because the kernel-based methods can only handle motions within the preset kernel size. As for the flow-based methods, they usually optimize the optical flow in a local patch iteratively, which has demonstrated its effectiveness in real-world cases. However, in a cartoon image, the optimal destination may locate outside the local patch due to large motions, and there are regions with similar colors in the patch. Therefore, the optimization of the optical flow can be easily trapped by the local minima.

To circumvent the local minima, we improve the optical flow estimation with a global matching strategy so that the flow is optimized within patches near the optimal destination. Specifically, we segment cartoon images into color pieces and globally match those pieces. Then, the global matching is converted to a coarse optical flow by the inter-piece deformation, and the coarse flow is treated as the guidance of a flow estimator. With the global matching, we propose a novel animation interpolation framework. Extensive experiments demonstrate our global matching strategy can effectively improve the optical flows of animation frames, and our method outperforms state-of-the-art (SOTA) interpolation methods on our dataset and generates better results with more details and objects reserved.

% FFF still falls into the flow-based category and is composed of a flow estimation module and a synthesis network to generate the intermediate frames. Differently, we involve global information in our flow module to alleviate the local minima. Specifically, we segment cartoon frames into color regions and match inter-frame regions with the similarity calculated by VGG \ref{} features. After rejecting false pairs by distance and size constraints, we attained the shift and deformation between two matchings by minimizing the warping energy function described in Sect.~\ref{}. Finally, we combined all valid matchings to weave a guidance flow as a compensation of our flow module. 

% ATD contains 12,000 triplets and is divided into two parts,  To ease the burden of human labor, we leveraged SSIM \ref{} and RAFT \ref{} to automatically filter invalid triplets with repeated frames and inconsistent motions. 



% Moreover, we as a baseline for this task.
% %
% We find, however, by simply finetuning the existing video interpolation algorithms.
% %
% To address this problem, we propose a . 
% %
% Specifically, we develop a XXX module based on global color piece matching, which can predict a guidance.
% %

% ATD contains 12,000 triplets and is divided into two parts, the training set ATD-10K with 10,000 triplets and the test set ATD-2K with 2,000 triplets. Those triplets were selected out of nearly one million candidates which are collected from 28 animation movies with a total length of 1,000 minutes. To ease the burden of human labor, we leveraged SSIM \ref{} and RAFT \ref{} to automatically filter invalid triplets with repeated frames and inconsistent motions. 

% is very difficult.
%

%

% We also p

% An effective animation video interpolation algorithm should  tackle the large motions for high-quality frame generation.


%
% From our respective, there are two distinctive characteristics in animation.
%


% One biggest gap is.

% Due to the lower frame rate, the motion between adjacent frames are generally larger than that of the real-world video
% Besides the data gaps, data collection is another issue of animation interpolation. 
% %
% So far, there is no suitable dataset for neither for training nor for evaluation.

% Due to the low frame rate and irregular motions of animations, sequential frames cannot be used to train or test interpolation models as existing datasets do, \eg, Adobe240 \ref{} and YouTube960 \ref{}. Instead, it is possible to collect valid triplets with smooth motions from animation videos, but there are only 3\% valid triplets on average.

% Video interpolation has been extensively studied in recently years. The relevant methods usually take advantage of deep learning and can be roughly classified into two categories, \ie, the kernel-based and the flow-based. Kernel-based methods \ref{} learn a large size kernel for each pixel and convolve the kernels with the input to generate the intermediate image. Flow-based methods usually estimate optical flows of the input images with off-the-shelf flow estimators like PWCNet \ref{}. Then, the intermediate frame is restored by a learning-based interpolation network. To get better results, the flow-based approaches also improved warping strategies, \eg, the depth-aware flow projection layer\ref{}, deformable warping \ref{}, and softmax splatting\ref{}, or employed high order motion models \ref{}. 




% \begin{figure}
% \centering
% \subfloat[]{%
% \label{fig:character_anime-a}
%   \includegraphics[width=.47\columnwidth]{figures/BingGuo_008795.jpg}%
%   \includegraphics[width=.47\columnwidth]{figures/BingGuo_008795.jpg}%
% }
% \quad
% \subfloat[]{%
% \label{fig:character_anime-b}
%   \includegraphics[width=.47\columnwidth]{figures/BingGuo_008795.jpg}%
%   \includegraphics[width=.47\columnwidth]{figures/BingGuo_008795.jpg}%
% }
% \caption{Characteristics of animations in appearance and motion. (a) displays the clear contours, flat blocks, simple textures. (b) shows statistics of animations and real-world videos.}
% \end{figure}

%\begin{figure} 
%   \centering
%   \begin{subfigure}{.47\columnwidth}
%       \centering
%       \includegraphics[width=\columnwidth]{figures/fig1_a.eps} \\
%       \includegraphics[width=\columnwidth]{figures/fig1_a.eps}
%       \caption{}\label{fig:1a}        
%   \end{subfigure}
%   \quad
%   \begin{subfigure}{.47\columnwidth}
%       \centering
%       \includegraphics[width=\columnwidth]{figures/fig1_b.eps}
%       \includegraphics[width=\columnwidth]{figures/fig1_b.eps}
%       \caption{}\label{fig:1b}
%   \end{subfigure}
%\caption{}
%\label{fig:}
%\end{figure}

% First, the appearance of animations is different from the common videos at least in three ways, namely, 1) Clear contours for objects or semantic parts. 2) Flat blocks filled with the same or closed colors. 3) Less textures and shades. As a result, trained on real-world sequences, learning-based interpolation methods poorly handle the reconstruction of the boundaries, color blocks and smooth textures of animations. We illustrate the differences between animations and real-world videos in Fig.~\ref{fig:character_anime-a} and provide failure cases generated by XXX\ref{} in Fig.~\ref{fig:failure_case-a}.




%it is hardly possible to collect a large amount of sequential frames with smooth motions as datasets for interpolation models as Adobe240 \ref{}. Even for triplets, there are only 2\% valid samples on average.

% \begin{figure}
% \centering
% \subfloat[]{%
% \label{fig:failure_case-a}
%   \includegraphics[width=.47\columnwidth]{figures/BingGuo_008795.jpg}%
%   \includegraphics[width=.47\columnwidth]{figures/BingGuo_008795.jpg}%
% }
% \quad
% \subfloat[]{%
% \label{fig:failure_case-b}
%   \includegraphics[width=.47\columnwidth]{figures/BingGuo_008795.jpg}%
%   \includegraphics[width=.47\columnwidth]{figures/BingGuo_008795.jpg}%
% }
% \caption{Failure cases of existing interpolation methods and flow estimators.}\label{fig:failure_case}
% \end{figure}

% To address the aforementioned problems, we make initial efforts towards the animation video interpolation in this paper. Firstly, we constructed an animation triplet dataset named ATD. ATD contains 12,000 triplets and is divided into two parts, the training set ATD-10K with 10,000 triplets and the test set ATD-2K with 2,000 triplets. Those triplets were selected out of nearly one million candidates which are collected from 28 animation movies with a total length of 1,000 minutes. To ease the burden of human labor, we leveraged SSIM \ref{} and RAFT \ref{} to automatically filter invalid triplets with repeated frames and inconsistent motions. 

% To address this problem, we propose a . 
%


%


% Secondly, 

% Besides the guidance flow, we also introduce the region aware importance to handle multiple pixels that are mapped to the same location in forward warp. To be specific, we calculate importance score maps by back warping image $\#1$ and $\#1$ in a triplet. Then, we propagate the scores along the segmented color blocks and finally treat those scores as a clue for depth in forward warp.

Our main contributions are summarized as follows:
\begin{itemize}
%\vspace{-2mm}
%\setlength{\itemsep}{0pt}
%\setlength{\parsep}{0pt}
%\setlength{\parskip}{0pt}
\item We construct a hard-to-collect benchmarking dataset called ATD for animation video interpolation. It contains 10,000 training triplets and 2,000 test triplets with diversified labels. To the best of our knowledge, ATD is the first animation triplet dataset in the field of video interpolation.
\item With ATD, we conduct thorough evaluations on the performance of recent interpolation methods on synthesizing animation frames. Be believe that the benchmarks will facilitate the follow-up researches in animation interpolation.
\item We propose a novel animation interpolation framework with a global matching strategy. The global matching helps the optimization of optical flow to avoid the local minima, and the proposed method achieves the best performance and can generate more contents that SOTA interpolation methods may miss.
\end{itemize}

